Linear-Scaling Selected Inversion based on Hierarchical Interpolative Factorization for Self Green's Function for Modified Poisson-Boltzmann Equation in Two Dimensions

This paper studies an efficient numerical method for solving modified Poisson-Boltzmann (MPB) equations with the self Green's function as a state equation to describe electrostatic correlations in ionic systems. Previously, the most expensive point of the MPB solver is the evaluation of Green's function. The evaluation of Green's function requires solving high-dimensional partial differential equations, which is the computational bottleneck for solving MPB equations. Numerically, the MPB solver only requires the evaluation of Green's function as the diagonal part of the inverse of the discrete elliptic differential operator of the Debye-H\"uckel equation. Therefore, we develop a fast algorithm by a coupling of the selected inversion and hierarchical interpolative factorization. By the interpolative factorization, our new selected inverse algorithm achieves linear scaling to compute the diagonal of the inverse of this discrete operator. The accuracy and efficiency of the proposed algorithm will be demonstrated by extensive numerical results for solving MPB equations.

==> figure/Level1_5.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{6.0cm}{!}{
\input{figure/fig-comp-modules/level1_5}
}


\end{minipage}
\caption{Level $3/2$}
\label{fig:lel1-5}
\end{figure}

==> figure/Level2_5.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{6.0cm}{!}{
\input{figure/fig-comp-modules/level2_5}
}


\end{minipage}
\caption{Level $5/2$}
\label{fig:lel2-5}
\end{figure}

==> figure/Level3_0.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{12.0cm}{!}{
\input{figure/fig-comp-modules/level2_5}
\input{figure/fig-comp-modules/level3_0}
}


\end{minipage}
\caption{Left: Level $5/2.$ Right: Level $3$}
\label{fig:lel3-0}
\end{figure}
